SYNCA: A Synthetic Cyclotron Antenna for the Project 8 Collaboration

Cyclotron Radiation Emission Spectroscopy (CRES) is a technique for measuring the kinetic energy of charged particles through a precision measurement of the frequency of the cyclotron radiation generated by the particle's motion in a magnetic field. The Project 8 collaboration is developing a next-generation neutrino mass measurement experiment based on CRES. One approach is to use a phased antenna array, which surrounds a volume of tritium gas, to detect and measure the cyclotron radiation of the resulting $\beta$-decay electrons. To validate the feasibility of this method, Project 8 has designed a test stand to benchmark the performance of an antenna array at reconstructing signals that mimic those of genuine CRES events. To generate synthetic CRES events, a novel probe antenna has been developed, which emits radiation with characteristics similar to the cyclotron radiation produced by charged particles in magnetic fields. This paper outlines the design, construction, and characterization of this Synthetic Cyclotron Antenna (SYNCA). Furthermore, we perform a series of measurements that use the SYNCA to test the position reconstruction capabilities of the digital beamforming reconstruction technique. We find that the SYNCA produces radiation with characteristics closely matching those expected for cyclotron radiation and reproduces experimentally the phenomenology of digital beamforming simulations of true CRES signals.

==> author.tex <==
%\newcommand{\mitt}{Laboratory for Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
%\newcommand{\mainz}{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, 55128 Mainz, Germany}
%\newcommand{\psu}{Department of Physics, Pennsylvania State University, University Park, PA 16802, USA}
%\newcommand{\cwru}{Department of Physics, Case Western Reserve University, Cleveland, OH 44106, USA}
%\newcommand{\ucsb}{Department of Physics, University of California, Santa Barbara, CA}
%\newcommand{\uw}{Center for Experimental Nuclear Physics and Astrophysics and Department of Physics, University of Washington, Seattle, WA 98195, USA}
%\newcommand{\pnnl}{Pacific Northwest National Laboratory, Richland, WA 99354, USA}
%\newcommand{\haystack}{Haystack Observatory, Massachusetts Institute of Technology, Westford, MA}
%\newcommand{\caltech}{California Institute of Technology, Pasadena, CA}
%\newcommand{\nrao}{National Radio Astronomy Observatory}
%\newcommand{\paris}{Laboratoire de Physique Nucl\'eaire et de Hautes \'Energies, Sorbonne Universit\'e, Universit\'e de Paris, CNRS/IN2P3, Paris, France}
%\newcommand{\yale}{Wright Laboratory, Department of Physics, Yale University, New Haven, CT 06520, USA}
%\newcommand{\llnl}{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}
%\newcommand{\iu}{Department of Physics, Indiana University, Bloomington, IN 47405, USA}
%\newcommand{\kit}{Institute for Astroparticle Physics, Karlsruhe Institute of Technology, 76021 Karlsruhe, Germany}

\author[a]{A.~Ashtari Esfahani} 
% \author[b]{Z.~Bogorad}
\author[c]{S.~B\"oser} 
\author[b]{N.~Buzinsky}
% \author[a]{R.~Cervantes} 
\author[d]{M.~C.~Carmona~Benitez}
\author[a]{C.~Claessens} 
\author[d]{L.~de~Viveiros}
%\author{S.~Doeleman} \affil{Harvard-Smithsonian Center for Astrophysics, Cambridge, MA 02138, USA}
\author[a]{P.~J.~Doe} 
\author[a]{S.~Enomoto} 
\author[c]{M.~Fertl}
\author[b]{J.~A.~Formaggio}
% \author[e]{L.~Gladstone}
%\author{M.~G\"odel}\affil{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, 55128 Mainz, Germany}
% \author[f]{J.~K.~Gaison} 
\author[f]{M.~Grando} 
% \author[a1,f]{M.~Guigue}
% \author[a]{J.~Hartse}
\author[g]{K.~M.~Heeger} 
\author[f]{X.~Huyan} 
% \author[b]{J.~Johnston} 
\author[f]{A.~M.~Jones} 
\author[h]{K.~Kazkaz}
% \author[f]{B.~H.~LaRoque} 
\author[b]{M.~Li}
\author[c]{A.~Lindman} 
\author[c]{C.~Matth\'{e}} 
\author[e]{R.~Mohiuddin} 
\author[e]{B.~Monreal} 
\author[d]{R.~Mueller}
\author[g]{J.~A.~Nikkel} 
\author[a]{E.~Novitski} 
\author[f]{N.~S.~Oblath} 
\author[b]{J.~I.~Pe\~{n}a}
\author[j]{W.~Pettus} 
\author[c]{R.~Reimann}
\author[a]{R.~G.~H.~Robertson}
\author[a]{G.~Rybka} 
\author[g]{L.~Salda\~na} 
% \author[b]{V.~Sibille} 
\author[f]{M.~Schram} 
\author[g]{P.~L.~Slocum}
\author[b]{J.~Stachurska}
\author[e]{Y.-H.~Sun}
\author[g]{P.~T.~Surukuchi}
\author[f]{J.~R.~Tedeschi} 
\author[g]{A.~B.~Telles}
\author[c]{F.~Thomas} 
\author[f]{M.~Thomas}  
\author[c]{L.~Thorne} 
\author[i]{T.~Th\"ummler} 
% \author[h]{L.~Tvrznikova} 
\author[b]{W.~Van~De~Pontseele}
\author[f,a]{B.~A.~VanDevender} 
%\author{J.~Weintroub} \affil{Harvard-Smithsonian Center for Astrophysics, Cambridge, MA 02138, USA}
\author[g]{T.~E.~Weiss} 
\author[d]{T.~Wendler} 
% \author[b]{E.~Zayas} 
\author[d, 1]{A.~Ziegler, \note{Corresponding author.}}

\affiliation[a]{Center for Experimental Nuclear Physics and Astrophysics and Department of Physics, University of Washington, Seattle, WA 98195, USA}
\affiliation[b]{Laboratory for Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{c}{Institut fur Physik, Johannes Gutenberg-Universitat Mainz, 55128 Mainz, Germany}
%\affiliation[d]{\psu}
%\affiliation[e]{\cwru}
%\affiliation[f]{\pnnl}
%\affiliation[g]{\yale}
%\affiliation[h]{\llnl}
%\affiliation[i]{\kit}
%\affiliation[j]{\iu}
%\affiliation[k]{\paris}
